D0 Top Quark Results and their Dependence on Successful Grid Computing

The heaviest known Fermion particle -- the top quark -- was discovered at Fermilab in the first run of the Tevatron in 1995. However, besides its mere existence one needs to study its properties precisely in order to verify or falsify the predictions of the Standard Model. With the top quark's extremely high mass and short lifetime such measurements probe yet unexplored regions of the theory and bring us closer to solving the open fundamental questions of our universe of elementary particles such as why three families of quarks and leptons exist and why their masses differ so dramatically. To perform these measurements hundreds of millions of recorded proton-antiproton collisions must be reconstructed and filtered to extract the few top quarks produced. Simulated background and signal events with full detector response need to be generated and reconstructed to validate and understand the results. Since the start of the second run of the Tevatron the D0 collaboration has brought Grid computing to its aid for the production of simulated events. Data processing on the Grid has recently been added and thereby enabled us to effectively triple the amount of data available with the highest quality reconstruction methods. We will present recent top quark results D0 obtained from these improved data and explain how they benefited from the availability of computing resources on the Grid.

==> ShortCuts.tex <==
% Daniels Shortcuts
%
%ArXiv directive:
%auto-ignore
%
\newcommand{\vektor}[2]
{{#1 \choose #2}}
%{\begin{array}[b]{c} 
%   \left( \displaystyle \begin{array}[b]{c}#1\\#2\end{array}\right) \\
% \end{array}
%}
\newcommand{\SU}{SU}
\newcommand{\SO}{SO}
\newcommand{\U}{U}

\newcommand{\hc}{\mbox{h.c.}}
\newcommand{\Tr}{\mbox{Tr}}

\newcommand{\PC}{Potenzreihenkorrektur}
\newcommand{\PCen}{Potenzreihenkorrekturen}

\newcommand{\Slash}[1]{\mbox{\it #1\hspace{-0.6em}\slash}}

\newlength{\ziffer}
\newcommand{\0}{\settowidth{\ziffer}{0}\hspace*{\ziffer}}

\newcommand{\TeV}{\,\mbox{Te\kern-0.2exV}}
\newcommand{\GeV}{\,\mbox{Ge\kern-0.2exV}}
\newcommand{\mGeV}{\,\mathrm{Ge\kern-0.2exV}}
\newcommand{\MeV}{\,\mbox{Me\kern-0.2exV}}
\newcommand{\keV}{\,\mbox{ke\kern-0.2exV}}
\newcommand{\eV}{\,\mbox{e\kern-0.2exV}}
\newcommand{\km}{\,\mbox{km}}
\newcommand{\m}{\,\mbox{m}}
\newcommand{\cm}{\,\mbox{cm}}
\newcommand{\mm}{\,\mbox{mm}}
\newcommand{\um}{\,\mbox{$\mathrm\mu$m}}
\newcommand{\fm}{\,\mbox{fm}}
\newcommand{\us}{\,\mbox{$\mathrm\mu$s}}
\newcommand{\hz}{\,\mbox{Hz}}
\newcommand{\ipb}{\,\mbox{pb}^{-1}}
\newcommand{\ifb}{\,\mbox{fb}^{-1}}
\newcommand{\pb}{\mbox{pb}}
\newcommand{\mb}{\mbox{mb}}

\newcommand{\bea}{\pagebreak[3]\begin{samepage}\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}\end{samepage}\pagebreak[3]}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}

\newcommand{\Bildzentriert}[3]
{  \begin{figure}[#2]
   \begin{center}
   \input #1
   \end{center}
   \caption{#3}
   \label{#1}
   \end{figure}
}

\newcommand{\Bild}[3]
{  \begin{figure}[#2]
   \input #1
   \caption{#3}
   \label{#1}
   \end{figure}
}

\newcommand{\C}{{C\hspace{-0.65em}I}}
\newcommand{\R}{{I\hspace{-0.35em}R}}
\newcommand{\N}{{I\hspace{-0.35em}N}}

\newcommand{\sm}{Standardmodell}
\newcommand{\ww}{Wechselwirkung}
\newcommand{\ee}{$e^+e^-$}
\newcommand{\as}{$\alpha_s$}
\newcommand{\Bmax}{B_{\mathrm{max}}}
\newcommand{\Bmin}{B_{\mathrm{min}}}
\newcommand{\Bsum}{B_{\mathrm{sum}}}
\newcommand{\Bdiff}{B_{\mathrm{diff}}}
\newcommand{\Mhigh}{M^2_{\mathrm{h}}/E^2_{\mathrm{vis}}}
\newcommand{\Mlow}{M^2_{\mathrm{l}}/E^2_{\mathrm{vis}}}
\newcommand{\Mhighp}{{M^{2 }_{(p)\mathrm{h}}}/E^2_{\mathrm{vis}}}
\newcommand{\Mlowp}{{M^{2}_{(p)\mathrm{l}}}/E^2_{\mathrm{vis}}}
\newcommand{\MhighE}{{M^{2}_{(E)\mathrm{h}}}/E^2_{\mathrm{vis}}}
\newcommand{\MlowE}{{M^{2}_{(E)\mathrm{l}}}/E^2_{\mathrm{vis}}}
\newcommand{\Mdiff}{M^2_{\mathrm{diff}}/E^2_{\mathrm{vis}}}
\newcommand{\durham}{{Durham}}

\newcommand{\met}{\slash\!\!\!\!{E_T}}

\newcommand{\ecm}{E_{\mathrm{cm}}}

\newcommand{\asb}{$\alpha_0$}

\newcommand{\eps}{\varepsilon}
\newcommand{\abb}{Fig.~\ref}
\newcommand{\fig}{\abb}
\newcommand{\tab}{Tab.~\ref}
\newcommand{\gl}[1]{Gl.~(\ref{#1})}
\newcommand{\eq}[1]{Eq.~(\ref{#1})}

\newcommand{\oas}{$\cal O$($\alpha_s^2$)}
\newcommand{\oass}{$\cal O$($\alpha_s^3$)}

\newcommand{\sprime}{{\sc Sprime}}
\newcommand{\pythia}{{\sc Pythia}}
\newcommand{\jetset}{{\sc Jetset}}
\newcommand{\ariadne}{{\sc Ariadne}}
\newcommand{\herwig}{{\sc Herwig}}
\newcommand{\excalibur}{{\sc Excalibur}}
\newcommand{\minuit}{{\sc Minuit}}
\newcommand{\zfitter}{{\sc Zfitter}}
\newcommand{\event}{{\sc Event}}

\newcommand{\lep}{{\sc LEP}}
\newcommand{\delphi}{{\sc Delphi}}
\newcommand{\alephh}{{\sc Aleph}}
\newcommand{\opal}{{\sc Opal}}
\newcommand{\ldrei}{{\sc L3}}
\newcommand{\sld}{{\sc SLD}}
\newcommand{\delana}{{\sc Delana}}
%\newcommand{\dstfix}{{\sc Dstfix}}
\newcommand{\dstana}{{\sc Dstana}}
\newcommand{\delsim}{{\sc Delsim}}
\newcommand{\Mini}{{\sc Mini}}
\newcommand{\phwmini}{{\sc PHWMini}}
\newcommand{\cargo}{{\sc Cargo}}
\newcommand{\jade}{{\sc Jade}}

\newcommand{\tsppm}{\hspace{\tabcolsep}$\pm$\hspace{\tabcolsep}}

\newenvironment{scaledlist}[0]{
                          \begin{flushleft}
                          \begin{list}{{$\bullet$}}{\setlength{\itemsep}{2ex plus0.2ex}
                          \setlength{\parsep}{0ex plus0.2ex}
                          \setlength{\labelwidth}{2em}}
                         }
                         {
                          \end{list}
                          \end{flushleft}
                         }

 \newlength{\howlong}
\newcommand{\strikeout}[1]{
 \settowidth{\howlong}{#1}%
 #1\unitlength0.5ex%
 \begin{picture}(0,0)
   \linethickness{0.35mm}
   \put(0,1.4){\line(-1,0){\howlong\divide\unitlength}}
 \end{picture}%
}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 

